Achieving Adversarial Robustness via Sparsity

Network pruning has been known to produce compact models without much accuracy degradation. However, how the pruning process affects a network's robustness and the working mechanism behind remain unresolved. In this work, we theoretically prove that the sparsity of network weights is closely associated with model robustness. Through experiments on a variety of adversarial pruning methods, we find that weights sparsity will not hurt but improve robustness, where both weights inheritance from the lottery ticket and adversarial training improve model robustness in network pruning. Based on these findings, we propose a novel adversarial training method called inverse weights inheritance, which imposes sparse weights distribution on a large network by inheriting weights from a small network, thereby improving the robustness of the large network.

==> LaTeX arXiv/Conclusion.tex <==
\section{Conclusion}

%As shown in Fig., the clean and adversarial accuracy will compromise simultaneously in almost every pruning settings. Thus comes the most counter-intuitive phenomenon in our results, on Tiny-ImageNet, the ResNet18 gains robustness improvement in the sacrifice of clean accuracy after unstructured pruning. However, we suggest that this phenomenon can be explained by the increasing complexity of the decision boundary in adversarial settings. (Fig.~\ref{fig:illustration_of_decision_boundary} provides an illustration)
%
%\begin{figure}
%\resizebox{.49\textwidth}{!}{
%\centering
%\includegraphics[width=\textwidth]{figures/boudary}
%}
%\caption{An illustration of decision boundaries of different networks. Left: The decision boundary of a network trained with clean examples. Middle: The decision boundary of an adversarially trained network. Right: The decision boundary of a \textbf{pruned} and adversarially trained network. As the complexity of separating the examples with $ L_\infty $ increases, the pruned network with restricted representation capacity may sacrifice thorny clean examples in reward of lower loss on adversarial examples.}
%\label{fig:illustration_of_decision_boundary}
%\end{figure}

% \YE{Consider rephrasing the conclusion after all results are updated}
We conduct comprehensive studies on adversarial network pruning. The contributions are three-fold: First, we give a new explanation on the connection between robustness and network sparsity, which is supported by much empirical evidence. 
% Second, we found out effective pruning methods and factors to obtain a robust network, including searching for the `winning ticket.' 
Second, we demonstrate the efficacy of training  network with robustness via our proposed algorithm including one-shot pruning and searching the `winning ticket.'
Third, we discover a new adversarial training strategy to achieve sparsity and large capacity at the same time for robustness.

%We conduct comprehensive studies on adversarial network pruning in this paper. With theoretical analysis and experiments on a variety of models and datasets, we find out the unique properties and challenges of network pruning in adversarial settings. Similar to natural models, `lottery ticket hypothesis' holds true for robust models, which enables us to efficiently prune a network at the early stage of adversarial training. Besides, the conventional training--pruning--fine-tuning pipeline implies higher robustness by automatic pruning in adversarial settings. In particular, the pruned network benefits from inherited weights by reaching a sparser weights distribution after retraining, which validates our theoretical analysis.
%In addition, we indicate the possibility of an increase in robustness while sacrificing clean accuracy when the network is pruned. Finally, we analyze that a large network can obtain higher clean accuracy and robustness than the pruned ones by proposing a new training strategy --- inverse weights inheritance --- which improves the overall performance of the model by impose sparser weights distribution, and also speeds up the adversarial training. We believe the findings are helpful and instructive in obtaining robust networks.



==> LaTeX arXiv/Introduction.tex <==
\section{Introduction}

It is widely recognized that deep neural networks (DNNs) are usually over-parameterized, and network pruning has been adopted to remove insignificant weights from a large neural network without hurting the accuracy. Despite its success, pruning strategies have been rarely discussed in the adversarial learning setting where the network is trained against adversarial examples, and the robustness of the network is as important as accuracy.

It is unclear what pruning methods are effective and which factors are critical for retaining model robustness. Believing that the inherited model weights may not be effective in preserving network accuracy \cite{DBLP:journals/corr/abs-1903-12561, DBLP:conf/iclr/LiuSZHD19}, \citet{DBLP:journals/corr/abs-1903-12561} propose a concurrent adversarial training and weight pruning framework to seek a compressed robust model. \citet{gui2019model} further incorporates pruning and several other techniques into a unified optimization framework to preserve high robustness while achieving a high compression ratio. However, the conventional three-stage `training--pruning--fine-tuning' pipeline has not been closely examined in the adversarial context. More crucially, it is unclear which components in the network pruning methods are critical to preserving model performance. To this end, we design a comprehensive set of experiments to answer these questions.

Despite some adversarial pruning methods that have been proposed, there is still a lack of theoretical foundation to explain the working mechanism behind those methods. In fact, there are seemingly contradictory opinions on the robustness of pruned networks: \citet{DBLP:conf/iclr/MadryMSTV18} suggests network capacity is crucial to robustness, and a wider network is more likely to obtain higher accuracy and robustness than a simple network. In contrast, \citet{guo2018sparse} theoretically proves that an appropriately higher weight sparsity implies stronger robustness on naturally trained models. Other theories such as the `Lottery Ticket Hypothesis' \cite{DBLP:conf/iclr/FrankleC19} point out that, a subnetwork extracted from a large network can always achieve comparable performance with the original one in the natural setting. However, it remains unknown if the hypothesis holds true for adversarially robust networks. We are motivated to explore how adversarial pruning affects the intrinsic characteristics of the network and its impact on model robustness.

In this study, we find that the robustness of the model improves as its weights become sparser. We show that weights sparsity not only includes the traditional $L_{0}$-sparsity, {\em i.e.}, the number of parameters retained, but also a weight distribution closer to zero, represented generally by the $L_{p}$ norm of weights. These forms of sparsity can lead to robustness improvement, which is verified theoretically and experimentally.
By extensive experiments on a variety of state-of-the-art pruning methods, models, and datasets, we also demonstrate that a pruned network inheriting weights from a large robust network has improved robustness than a network with the same structure but randomly initialized weights. Moreover, weight inheritance implicitly produces sparser weights distributions on adversarially pruned models.

Inspired by the connection between model sparsity and robustness, we propose a new adversarial training strategy called {\em Inverse Weights Inheritance}: by inheriting weights from a pruned model, a large network can achieve higher robustness than being adversarially trained from scratch. The pruned model can be the `winning ticket' of the large network, as we verify that `Lottery Ticket Hypothesis' \cite{DBLP:conf/iclr/FrankleC19} holds true in the adversarial learning context. The performance results of our proposed training strategy corroborate that sparse weights and high capacity are not contradictory, but contribute joint efforts to model robustness.

The contributions of the paper can be summarized as follows. {\em First,} we establish the theoretical connection between network robustness and sparsity. {\em Second,} through comprehensive experiments, we find that weights inheritance and adversarial training are important in adversarial pruning, and implicitly provide weights sparsity. {\em Finally,} we propose a new adversarial training strategy that achieves improved robustness.

\begin{figure}[t]
	\centering
% 	\includegraphics[width=0.85\columnwidth]{figures/nparam.pdf}
	\includegraphics[width=0.8\columnwidth]{figures/nparam0.pdf}
	\caption{The relation between parameter numbers and adversarial robustness in our approach and the state-of-the-art methods on different architectures. The dotted lines represent the baselines of three base (large) models. Models residing at the upper left corner have higher adversarial accuracies and smaller sizes. All models are adversarially trained by PGD with $ \epsilon = 8/255 $ and 10 steps, and evaluated by PGD attack of $ \epsilon = 8/255 $ and 100 steps on CIFAR10. We also mark the results \citet{Guo2020} and \citet{gui2019model} by stars in the same settings. Our experiments show that adversarial pruning methods are effective in obtaining networks of smaller parameters with comparable or even better robustness than the baselines.} 
	\label{fig:nparam}
\end{figure}

\iffalse
%Most pruning methods follow the `training--pruning--fine-tuning' pipeline, and can be roughly categorized by whether the pruning 1) is iterative or one-shot, 2) focuses on a local region or the entire model, and 3) is structured or not. With the particular library and hardware support, the pruned model can be deployed to resource-constrained devices with little accuracy loss.

%leading to  unnecessary storage and  on storage and . In order to mitigate this problem, neural network pruning is proposed. Until now, various kinds of pruning methods are designed and studied. The basic pruning principles can be divided into the following categories: iterative and one-shot, local and global, and structured and unstructured pruning. While unstructured pruning requires specific library and hardware support, structured pruning can directly decrease the capacity of the network and the inference overhead. With the success of network pruning algorithms in a wide range of domains, the computational paradigm could be shifted from powerful cloud to thin mobile devices with limited resources, which also pose as vulnerable attack surfaces of adversarial examples.


Different from natural settings, model performance is evaluated by both clean accuracy (accuracy on the clean data) and robustness (accuracy on the adversarial data) in adversarial settings. Moreover, as adversarial training introduces significant computation overhead, there is a pressing need for pruning at the earlier stages. Some preliminary efforts in this aspect have been made:
\cite{wang2018adversarial} indicates that when pruning is applied, robustness drops earlier than clean accuracy.
\cite{DBLP:journals/corr/abs-1903-12561} strengthens the benefit of inherited weights in adversarial settings by showing that a small network can preserve performance through concurrently pruning and training.
\cite{zhao2018compress} investigates the transferability of adversarial examples between uncompressed and compression models, and finds adversarial examples at high sparsity are marginally less transferable in natural settings.

In this work, we theoretically and empirically reveal properties of network pruning in adversarial settings, which may or may not hold in natural settings. Based on extensive experiments on a variety of state-of-the-art pruning methods, models, and datasets, we have the following interesting findings. {\em First}, `winning ticket' exists in robust models, and can be found efficiently by iterative pruning, {\em i.e.}, `lottery ticket hypothesis' \cite{DBLP:conf/iclr/FrankleC19} holds true in adversarial settings.
%{\em Second}, we demonstrate the possibility to automatically compress a robust model without performance loss. In some cases, we even observe an improvement in robustness after pruning, which is not observed in \cite{wang2018adversarial,gui2019model,ye2018rethinking}. On the contrary, inherited weights by predefined structured pruning \cite{DBLP:conf/iclr/0022KDSG17} does not enhance performance on robust models, sharing a similar conclusion in the natural setting \cite{DBLP:conf/iclr/LiuSZHD19}.
{\em Second}, we demonstrate the inherited weights by automatic pruning imply higher weights sparsity and lead to higher robustness than the same small networks trained from scratch. We even observe an improvement in robustness after pruning, which is not observed in \cite{wang2018adversarial,gui2019model,ye2018rethinking}. On the contrary, inherited weights by predefined structured pruning \cite{DBLP:conf/iclr/0022KDSG17} does not enhance performance on robust models, sharing a similar conclusion in the natural setting \cite{DBLP:conf/iclr/LiuSZHD19}.
{\em Third}, we reveal that models with weights distribution closer to zero imply higher robustness theoretically and empirically by providing a new adversarial training method called {\em Inverse Weights Inheritance}. Higher $L_0$-sparsity, namely, network pruning can be viewed as a special case to force smaller weights distribution. Thus a large network has the capability to attain higher accuracy and robustness than the pruned ones.

%    Overall, we made the following contributions. To the best of our knowledge, this work is among the first conducting comprehensive experiments on adversarially robust network pruning, covering a wide range of pruning methods, training approaches, models, and datasets. Drawn on the results, we concur or challenge pruning properties proposed in previous works, in adversarial settings or not. In light of these properties, we show effective ways to obtain small robust models, and to improve the performance of a large robust model.
\fi


==> LaTeX arXiv/Proof.tex <==
\section{Proof of Theorem 3.2}
	Let us denote layer-wise activation output as $ a_0=x $ and $ a_j = \sigma \left( W_j^T a_{j-1} \right) $ for $ 0 \le j \le d-1 $. We also define $ D_j $ as
    \begin{equation}
        \label{equation:activation}
            D_j\left(x\right) := diag \left( 1_{W_j[:,1]^T a_{j-1}>0}, ..., 1_{W_j[:,n_j]^T a_{j-1}>0} \right)
    \end{equation}
    which is a diagonal matrix whose entries will take value one when the activation is nonzero within $j$-th layer. Note that if for any $x$ and any $j \in \{1,...,d-2\}$, $D_j(x)=0^{n_j \times n_j}$, $D_{d-1}(x)=0^{n_{d-1} \times n_{d-1}}$ must hold. In this setting, we have Lemma \ref{lemma:lipschitz_sparsity_with_D} proved by \cite{guo2018sparse}.

    \begin{lemma}
        \label{lemma:lipschitz_sparsity_with_D}
        (A local Lipschitz constant for ReLU networks \cite{guo2018sparse}) Letting $\frac{1}{p}+\frac{1}{q}=1$, for any $x \in \mathbb{R}^n $, $k \in \{1,...,c\}$ and $q \in \{1,2\}$, the local Lipschitz constant of function $ g_{\hat{y}}\left(x\right)-g_k\left(x\right) $ satisfies
        \begin{equation}
        \label{equation:lipschitz_sparsity_with_D}
            L^k_{q,x} \le \left\Vert w_{\hat{y}}-w_k \right\Vert_q\sup_{x'\in B_p\left(x,R\right)}\prod_{j=1}^{d-1}
            \left( {\left\Vert D_j\left(x'\right) \right\Vert_p} {\left\Vert W_j \right\Vert_p} \right)
        \end{equation}
        where all the matrix norms are induced norms.
    \end{lemma}

    In our settings, the network is pruned to avoid layer removal and thereby for any $j \in [0, d-1]$, $W_{j}$ cannot be all-zero matrices. Then we prove for any $j \in [0, d-1]$, there must be at least one $a_{j}$ which is not an all-zero matrix. We prove that by contradiction. Assume that for layer $j$, $a_{j}$ is an all-zero matrix. Then $D_{j}(x) = 0^{n_{d-1} \times n_{d-1}}$ which yields $D_{d-1}(x)=0^{n_{d-1} \times n_{d-1}}$ and the prediction score $g_k(x)$ will be all-zero for any $k$ since 
    \begin{equation}
        \label{equation:perceptron}
            g_k\left(x_i\right) = w_k^T \sigma \left(W_{d-1}^T \sigma \left( ... \sigma \left( W_1^T x_i\right) \right) \right).
    \end{equation}
    It is impossible for a well-trained network to make all-zero predictions, which leads to a contradiction. Hence the assumption is not true and $a_{j}, \forall j\in [0, d-1] $ cannot be an all-zero matrix. The conclusion implies that, for any $j\in [0, d-1]$, there must be at least one entry in $ D_{j}(x) $ taking the value $1$. By the definition of matrix induced norms, we have that for any $x$ and particular values of $p$,
    \begin{equation}
        \label{equation:L_2_norm}
        \left\Vert D_j\left(x\right) \right\Vert_2 := \sigma_{\max}(D_j) = 1
    \end{equation}
    \begin{equation}
        \label{equation:L_inf_norm}
        \left\Vert D_j\left(x\right) \right\Vert_\infty := \max_{1\le i \le n_j}\sum_{m=1}^{n_j}\vert D_j[i,m]\vert = 1
    \end{equation}
    where $\left\Vert D_j\left(x\right) \right\Vert_2$ is the spectral norm, the greatest singular value of $D_j\left(x\right)$. Then for $p = 2$ and $\infty$, the right side of Eq.~\eqref{equation:lipschitz_sparsity_with_D} is independent of input $ x $ and we have the relation between the Lipschitz constant and weight sparsity described by Theorem 3.2.

==> LaTeX arXiv/RelatedWork.tex <==
% wangshufan edit 2020/01/09/18:45
\section{Related Work}

% Shufan Wang: Not sure whether to delete this part

% With the development of algorithms and network architectures, machine learning has become successful in lots of areas covering image classification, speech recognition, etc. However, state-of-the-art performance always comes with the burden of growing network capacity and training and inference overhead. In order to mitigate this problem, different compression methods are proposed, including network pruning, knowledge distillation and weights quantization, where network pruning is widely implemented because of its excellent performance and plasticity in practice.
\subsubsection{Adversarial Training.} Adversarial training and its variants are proposed to improve network robustness against adversarial examples \cite{DBLP:conf/iclr/KurakinGB17}. \citet{DBLP:conf/iclr/MadryMSTV18} motivates projected gradient descent (PGD) as a universal `first-order adversary,' and optimizes the saddle point formulation to train a robust network. \citet{DBLP:journals/corr/abs-1905-09747} observes robustness can transfer between networks by knowledge distillation, and such transfer can even improve the robustness of the student network. Following the convention, we adopt $L_\infty\text{-PGD}$ attack \cite{DBLP:conf/iclr/MadryMSTV18}, {\em i.e.,} the strongest attack utilizing the local first-order information of the network, both in adversarial training strategy and the robustness evaluations.

\subsubsection{Network Pruning Methods.} Network pruning methods related to this paper can be divided into two categories: structured pruning and unstructured pruning. Structured pruning prunes a network at the level of filters \cite{DBLP:conf/ijcai/2018,DBLP:conf/iclr/0022KDSG17,DBLP:conf/iccv/LuoWL17}, channels \cite{DBLP:conf/iccv/LiuLSHYZ17} or columns \cite{wen2016learning}, depending on their respective importance. %For filter pruning and channel pruning, the filters or output channels of a convolutional layer are pruned.
The importance of a filter or a channel can be determined by the norm of the weights \cite{DBLP:conf/iclr/0022KDSG17} or the channel scaling factor \cite{ye2018rethinking,DBLP:conf/iccv/LiuLSHYZ17} (sometimes the scaling factor in batch normalization layers). The unstructured pruning \cite{lecun1990optimal,hassibi1993second} prunes at the level of individual weight according to the Hessian matrix of the loss function. \citet{DBLP:journals/corr/HanPTD15} proposes to prune weights with small magnitude, and the compression ratio is further enhanced in \citet{DBLP:journals/corr/HanMD15} by quantization and Huffman coding. By incorporating non-negative stochastic gates, \citet{louizos2017learning} turns network pruning into an optimization problem with $ L_0 $-norm regularization. We pick representative structured and unstructured pruning methods to implement in our experiments. 

\subsubsection{Network Pruning in Adversarial Context.} Network pruning in adversarial context has been recently discussed in search of small and robust models \cite{wang2018adversarial,zhao2018compress,DBLP:journals/corr/abs-1903-12561,Sehwag2019}.
Several frameworks \cite{rakin2019robust,Madaan2019,gui2019model} have been proposed to adversarially train a neural network while constraining its size by pruning and/or quantization. 
% \citet{rakin2019robust} designs a multi-objective mechanism incorporating noise injection, lasso weight penalty and adversarial training to obtain small and robust networks. 
However, these works do not answer which pruning factors are important for robust networks, nor which pruning methods are effective.
%the optimization algorithms mentioned above neither explain why pruning works in adversarial settings, nor answer if a large network can be more robust than a pruned one. These key problems are discussed and figured out in our work.
%\cite{wang2018adversarial} also studies pruning in an adversarial setting, and indicates when pruning is applied, robustness drops earlier than clean accuracy. We will their observation does not always hold by a larger scale of experiments.

The `lottery ticket hypothesis' \cite{DBLP:conf/iclr/FrankleC19} shows the existence of a sparse subnetwork (or `winning ticket') in a randomly initialized network that can reach comparable performance with the large network. Nevertheless, \citet{DBLP:journals/corr/abs-1903-12561} argues against the existence of `winning ticket' in adversarial settings. On the other hand, \citet{Cosentino2019} manages to acquire adversarial winning tickets of simple models without harming model robustness. 
\citet{li2020towards} further proposed an optimized learning rate schedule to boost the searching performance of lottery tickets, while demonstrating why \citet{DBLP:journals/corr/abs-1903-12561} fails to find them. 

\citet{DBLP:conf/iclr/LiuSZHD19} claims that for network pruning in the natural setting, weights inherited by unstructured and predefined structured pruning may not be useful, as it may trap the pruned network to bad local minima. We show with experiments that weight inheritance improves the robustness in the adversarial setting, which we conjecture that this is because the inverse weights inheritance embrace larger networks during training, which can help jump out of local minima and achieve better generalization performance. \citet{hein2017formal} proposes a formal guarantee of adversarial robustness in terms of the local Lipschitz constant. By building a bridge between the local Lipschitz constant and weight sparsity, \citet{guo2018sparse} considers that an appropriately higher weight sparsity on naturally trained networks implies higher robustness. \citet{dinh2020sparsity} also finds an adversarially trained network with sparser weights distribution tends to be more robust, such as EnResNet20 \cite{wang2019resnets}. Different from compression, \citet{dhillon2018stochastic} proposes dynamic sparsity as an approach to improve robustness. By supplementing the concept of `sparsity,' we found empirical evidence of the link between robustness and sparsity, as well as training strategies to boost robustness.

%\textbf{Adversarial examples} are generated by adding imperceptible perturbations to the input which leads to misclassification. Successful attacks are thoroughly studied in prior researches such as FGSM \cite{DBLP:journals/corr/GoodfellowSS14}, PGD \cite{DBLP:conf/iclr/MadryMSTV18}, Deepfool \cite{DBLP:conf/cvpr/Moosavi-Dezfooli16}, and C\&W \cite{DBLP:conf/sp/Carlini017}. A PGD adversary can generate adversarial examples leveraging the gradients information with multi-step and random initialization. Defenses to adversarial examples are also well-studied. The major solutions include adversarial training \cite{DBLP:conf/iclr/MadryMSTV18} and its derivatives \cite{DBLP:conf/icml/ZhangYJXGJ19}, denoised networks \cite{DBLP:conf/cvpr/LiaoLDPH018}, and input transformation\cite{DBLP:conf/iclr/XieWZRY18} and reconstruction \cite{DBLP:conf/cvpr/SunTLYS19}. Adversarial training \cite{DBLP:conf/iclr/MadryMSTV18} is widely used because it is the most successful defense approach so far. By solving the min-max optimization problem, the network obtains a notion of security towards all first-order adversaries.

%\begin{equation}
%\label{eq:advtrain}
%\min_{\theta}\rho\left(\theta\right)=\mathbb{E}_{\left(x,y\right)\sim D}\left[\max_{\delta\in S}L\left(\theta, x+\delta, y\right)\right]
%\end{equation}
%
%\begin{equation}
%\label{eq:advgen}
%x^{t+1}={\prod}_{x+S}\left(x^{t}+\alpha sgn\left(\bigtriangledown_{x}L\left(\theta,x,y\right)\right)\right)
%\end{equation}


==> LaTeX arXiv/story/Experiment.tex <==
\section{Study of Robustness and Network Pruning}
\label{section:theory}

%In this section, we study the theoretical link between robustness and network sparsity, and explore by experiments effective pruning methods for robust networks. Posterior examination results support our theory and also suggest new ways for training robust networks.


%In this section, we first show that automatic network pruning may improve network robustness by imposing higher sparsity \textbf{(Sparsity in the following indicates a weights distribution closer to zero besides $L_0$-sparsity.)} Then we verify the `lottery ticket hypothesis' in adversarial settings. And finally, we propose a training strategy {\em Inverse Weight Inheritance}, through which a large network can obtain a sparser weights distribution and achieve higher robustness.
\input{story/theory}

\section{Performance Evaluation}
\label{section:experiment}

\input{story/implement}

\input{story/advprune}

\input{story/lottery}

\input{story/iwi}




==> LaTeX arXiv/story/advprune.tex <==

% Shufan Wang delete
%\par One more interesting finding is that, post adversarial pruning by global unstructured pruning or network slimming may directly lead to a robust and compact network without fine-tuning. This is not underlined in previous work. And this attribute may be useful in run-time network compression.

%Considering several models with similar performance on $ g_{\hat{y}}(x)-g_k(x) $, it is obvious that the model with weights distribution closer to zero tends to obtain a lower $L^k_{q,x}$ and higher robustness, regardless of whether it is a large model or a pruned one. Thus we get two hypotheses: 1)pruning can be viewed as a special approach to find weights distribution with higher $L_p$-sparsity, and appropriate pruning may lead to higher robustness. 2) For networks with same architecture, the network with sparser weights distribution tends to be more robust.

\subsection{Adversarial Network Pruning Improves Robustness by Imposing Higher Sparsity}
\label{section:story_1}

\begin{figure*}[t]
	\centering
% 	\resizebox{1.\linewidth}{!}{
% 	\includegraphics[width=\linewidth]{figures/inherit_reset_6.pdf}
	\includegraphics[width=1.0\linewidth]{figures/weight_distribution_reset_inherit_resnet18_half.pdf}
% 	}
	\caption{Weights distribution of the pruned network adversarially trained with \textbf{inherited weights} or \textbf{randomly initialized} weights. In general, networks with inherited weights from automatic pruning methods including LUP, GUP, NS have an equivalent or higher sparsity than their counterparts with randomly initialized weights. FP has lower sparsity than FP-rand.}
	\label{fig:weight_distribution_reset_inherit}
\end{figure*}

Although Thm.~\ref{theorem:lipschitz_sparsity} establishes a preliminary link between sparsity and robustness, it does not tell us how to achieve sparsity and therefore robustness by the equation. An intuitive way is to prune a network to reduce the number of non-zero weights of the model, which is also done in \cite{guo2018sparse} but only in the natural setting. We show in the following that pruning also works in the adversarial setting. Beyond that, we found that adversarial retraining after pruning mostly improves robustness, at a sparser weights distribution than models with the same structure.

We first adversarially train each base network until reaching the state-of-the-art clean and adversarial accuracy, and then prune each network by different means. 
\iffalse
When networks are pruned, we immediately test their accuracies on clean and adversarial samples. The results on CIFAR-10 and Tiny-ImageNet are shown in Table~\ref{table:accuracy_without_retrain2}. Please refer to the supplementary material for the results on CIFAR-100. Compared to the performance on the base network (marked under the model name), the pruned network only moderately suffers from accuracy loss when the pruning ratio is not very high, and the pruning methods are automatic, {\em i.e.,} LUP, GUP, and NS. Note that those methods automatically extract a subnetwork without altering the weights, resulting in a higher $L_0$ sparsity compared to base models. Considering pruning reduces model capacity, the mild performance loss is reasonable.
\fi

Although pruning shows a promising method to introduce sparsity, it does not end up in robust models each time. We hence impose adversarial retraining on pruned networks to enhance robustness. The results are provided in Table~\ref{table:advcom_three_datasets}. Since there is a tradeoff between accuracy and robustness \cite{DBLP:conf/icml/ZhangYJXGJ19}, and some models tend to sacrifice one for the other, we choose to report the performance where the sum of adversarial accuracy and clean accuracy is the highest. Distortion bound is also reported for a complete view. We refer readers to the supplementary material for further discussions on the results.

\input{tables/compare_prune_and_scratch100}

Most networks in Table~\ref{table:advcom_three_datasets} obtain higher accuracy and robustness than pruning without retraining, and a large proportion of them can achieve better performance than the base networks. Specifically, LUP and NS only suffer notable performance degradation at high pruning ratios, whereas GUP remains a remarkable high performance across all pruning ratios. FP cannot preserve network performance well.

To see whether the weights inherited from a large network help the pruned network converge, we conduct a series of comparison experiments, as shown in Table~\ref{table:compare_prune_and_scratch}. Compared to FP, FP-rand initializes a small network with the same structure as the corresponding pruned network. For automatic pruning methods including LUP, GUP, and NS, we re-use the pruned network structure with re-initialized weights. As we found, compared with FP-rand, FP provides little or no improvement with the inherited weights. On the contrary, automatic pruning with inherited weights almost always performs better than that with randomly initialized weights.

Although Table~\ref{table:advcom_three_datasets}, and Table~\ref{table:compare_prune_and_scratch} experimentally found effective methods or factors to gain robustness for pruned networks, it still remains unclear how it relates to sparsity. Interestingly, by examining the weights distribution after adversarial retraining, we found that most automatically pruned networks with inherited weights have similar or higher sparsity than those with randomly initialized weights, as some examples shown in Fig.~\ref{fig:weight_distribution_reset_inherit}, while the networks pruned by predefined pruning (FP) show the opposite trend. This could be explained by Thm.~\ref{theorem:lipschitz_sparsity}, since a weight distribution closer to zero implies higher robustness. Therefore, weight inheritance and adversarial retraining implicitly provide a way to obtain sparse networks. % Supplementary material contains more weights distribution visualization.

\subsubsection{Comparison with previous results.}
We also compare our conclusion with previous works and summarize the difference as follows. We find inherited weights by automatic pruning (LUP, GUP, NS) provide better initialization for small networks, while predefined pruning does not. \citet{DBLP:conf/iclr/LiuSZHD19} argues that weights inherited from structured pruning have little impact on the performance of the pruned network. While the experiments on FP agree with the conclusion, that on NS does not. \citet{wang2018adversarial} also suggests inherited weights are important to preserving network accuracy and robustness in adversarial settings, but they do not discuss the working mechanism behind. %But we disagree with \cite{DBLP:journals/corr/abs-1903-12561} on that post adversarial pruning fail to retain robustness, mainly because they only applied layer-wise pruninng, not global pruning in their work.

%Some may argue the legitimacy of the accuracy results we choose to report, as it has been pointed out that a trade-off exists between accuracy and robustness \cite{DBLP:conf/icml/ZhangYJXGJ19}. In fact, the trade-off does not affect our conclusions, but to resolve the concern, we display them in detail in the supplementary material.

%As we analyze, from the perspective of robust features \cite{ilyas2019adversarial}, it is likely that ResNet18 has limited capacity to express all features in Tiny-ImageNet, and it prefers to express more robust than non-robust features. That may inspire us to design more compact network architectures with higher robustness in the future.


==> LaTeX arXiv/story/implement.tex <==
\subsection{Implementation Details}

In this part, we describe the implementation details in examining adversarially robust network pruning. To obtain objective results, we mostly follow the experimental settings in previous works \cite{DBLP:conf/iclr/LiuSZHD19,DBLP:conf/icml/YangZXK19,DBLP:journals/corr/abs-1903-12561,DBLP:conf/icml/ZhangZ19}. Our experiments are carried out with PyTorch 1.0 on NVIDIA GeForce 2080 Ti GPUs.

\subsubsection{Datasets and Networks.} For the fairness of the results, we conduct experiments on CIFAR-10, Tiny-ImageNet, and CIFAR-100, which are representatives for small-scale datasets, large-scale datasets and datasets somewhere in between. Three state-of-the-art network architectures are chosen: VGG \cite{DBLP:journals/corr/SimonyanZ14a}, ResNet \cite{DBLP:conf/cvpr/HeZRS16}, and DenseNet \cite{DBLP:conf/cvpr/HuangLMW17} as the base large networks. A DenseNet-BC with depth $40$ and growth rate $k=12$ is also used. 

\subsubsection{One-Shot Pruning Methods.} We pick four representative and intrinsically different pruning methods: Global Unstructured Pruning (\textbf{GUP}) \cite{DBLP:conf/iclr/FrankleC19}, Local Unstructured Pruning (\textbf{LUP}) \cite{DBLP:journals/corr/HanMD15}, Filter Pruning (\textbf{FP}) \cite{DBLP:conf/iclr/0022KDSG17} and Network Slimming (\textbf{NS}) \cite{DBLP:conf/iccv/LiuLSHYZ17}. LUP and GUP are unstructured pruning, whereas FP and NS are structured pruning. Both GUP and NS prune globally according to the importance of weights or channels across all convolutional layers, while LUP and FP prune an identical percentage of weights or filters per layer locally. FP is a predefined pruning method while GUP, LUP and NS are automatic pruning methods where the structure is determined by the pruning algorithm at runtime.

We conduct these pruning methods in a one-shot manner that removes the parameters at one step, followed by post retraining to convergence. For all pruning methods, we re-implement each to achieve comparable performance with that reported in the current literature. For FP in ResNet, we conduct it on every two consecutive convolutional layers and skip the shortcuts according to \cite{DBLP:conf/iccv/LuoWL17}, also it is not available on DenseNet as pruning one filter would lead to input channel changes in all subsequent layers \cite{DBLP:conf/iclr/0022KDSG17,DBLP:conf/iclr/LiuSZHD19}. For NS, the highest pruning ratio is selected according to the maximum channel pruning ratio to avoid the removal of layers \cite{DBLP:conf/iccv/LiuLSHYZ17}.

\input{tables/advcom_three_datasets100}

\subsubsection{Adversarial Training and Evaluation.} We employ the widely used $ L_\infty\text{-PGD} $ adversary with $ \epsilon = 8/255, \text{step size} = 2/255 $ in our experiments. Following recent works \cite{Guo2020}, we utilize $ \text{iteration} = 10 $ for adversarial training, and evaluate robustness on $ \text{iteration} = 100 $. For all trainings, we adopt a SGD optimizer with momentum of $ 0.9 $ and weight decay of $ 5\times 10^{-4} $. The batch sizes for CIFAR-10 and CIFAR-100 are both $128$. On Tiny-ImageNet, the batch size is $128$ for ResNet18 and $32$ for DenseNet121 following \citet{DBLP:conf/icml/ZhangZ19} and \citet{DBLP:conf/icml/YangZXK19}. The distortion bound of adversarial examples \cite{bastani2016measuring, salman2019convex} also serves as a robustness metric, which is estimated by searching the minimum PGD $\epsilon$ that crafts a valid adversarial image on a given batch. We report the average of distortion bounds across all samples.

% Despite accuracy on clean and adversarial examples, the distortion bound of adversarial examples \cite{bastani2016measuring, moosavi2016deepfool, salman2019convex} also serves as a robustness metric, which is estimated by searching the minimum $\epsilon$ of PGD attack that crafts a valid adversarial image on a given batch of samples. We report the average of such distortion bounds across all batches.

%\cite{bastani2016measuring} evaluates the adversarial perturbation by a linear programming algorithm. \cite{moosavi2016deepfool} also utilizes average minimal perturbation on fixed data and error rates to compare various attack methods. \cite{salman2019convex} searches the bound of minimum adversarial distortion by different certifications, which represent the radius of the largest distortion ball that adversarial examples cannot exist. In our work, the distortion bound is estimated by finding the minimal $\epsilon$ of PGD attack that crafts a valid adversarial image in a given batch of samples. The actual average adversarial bound is calculated on multiple batches, which are the same in each run of testing.

\subsubsection{Stopping Criteria.} Typically, it is not well-defined how to train models to `full convergence' when stepwise decaying learning rate schedule is applied. Hence we adopt two stopping criteria indicating models have been sufficiently trained for ease of comparison. \textbf{Stop-E} denotes the network is trained for a fixed number of epochs. For CIFAR-10, CIFAR-100, and Tiny-ImageNet, we set the start learning rate to be $0.1, 0.1,$, and $0.01$, respectively. The learning rate is divided by $ 10 $ for every $1/3$ of the total epochs. \textbf{Stop-C} monitors the validation loss changes to automatically adjust the learning rate. For example, if we define patience to be $ 10 $ epochs and relative threshold to be $ 10^{-5} $, the learning rate only decays when the average validation loss does not decrease by more than $ 0.001\%$ for consecutive $10$ epochs. Models stop training after $2$ learning rate decays.


==> LaTeX arXiv/story/iwi.tex <==
% \input{tables/iwi100}

\begin{figure*}[t]
	\centering
% 	\resizebox{1.\linewidth}{!}{
	\includegraphics[width=\textwidth]{figures/iwi_weight_distribution.pdf}
% 	}
	\caption{ Weights distribution of large networks trained by \textbf{Inverse Weights Inheritance (IWI)} and adversarially trained with \textbf{random initialization (Baseline)}. Net XX\% denotes a large network trained by inheriting the weights of a `winning ticket' with XX\% weights pruned.}
	\label{fig:weight_distribution}
% 	\vspace{-3mm}
\end{figure*}

\begin{algorithm}[!b]
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\caption{Inverse Weights Inheritance (w/ Lottery Ticket)}
	\fontsize{9.5pt}{10.5pt}\selectfont
	\label{alg:iwi}
	\begin{algorithmic}[1] %[1] enables line numbers
		\REQUIRE \{$ f \left(x;\theta_0\odot M_0\right)$, $ p\% $, $ K $, $ N $\} same as in Alg.~\ref{alg:lottery_ticket}. \\
		~~~~~ Adversarial fine-tuning epochs $ N_f $.
		\ENSURE A robust network $ f \left(x;\theta''\right) $.
		\STATE {Find the winning ticket $ f \left(x;\theta_0\odot M_K\right) $ by Alg.~\ref{alg:lottery_ticket}.}
		\STATE {Adversarially fine-tune the `winning ticket' for $ N_f $ epochs, obtain a robust small network $g \left(x;\theta'\odot M_K\right)$.}
		\STATE {Load the weights of the pruned network $g$ to the corresponding place in the large network $f$ and obtain $f \left(x;\theta'\odot M_K\right).$}
		\STATE {Re-initialize weights of $f$ as $f \left(x;\theta'\odot M_K+\theta_{0} \odot \left(M_0-M_K\right)\right).$}
		\STATE{Train $f$ until convergence and obtain $ f \left(x,\theta''\right) $.}
		\STATE{\textbf{return} $ f \left(x;\theta''\right) $.}
	\end{algorithmic}
\end{algorithm}

\subsection{Inverse Weights Inheritance}
According to our experimental results in one-shot adversarial pruning, it seems that networks with smaller capacities (higher $L_0$-sparsity) can also have an equivalent or even higher accuracy and robustness than large networks. This appears to be contradictory to the conclusion in \citet{DBLP:conf/iclr/MadryMSTV18} that classifying examples in a robust way requires the model to have a larger capacity, as the decision boundary is more complicated. We ask the question that, {\em can a network be sparse and have larger capacity at the same time?} As we analyze, it is indeed possible to have such networks with superior performance.

We introduce a new training strategy called {\em inverse weights inheritance} (\textbf{IWI}), which is inspired by Thm.~\ref{theorem:lipschitz_sparsity} and adversarial network pruning results. By the strategy, a large network acquires sparse weights distribution by inheriting weights from a small robust network, which is pruned from the same large network in the first place and is adversarially trained. Alg.~\ref{alg:iwi} gives an example of using the lottery ticket to obtain such a small network. For a fair comparison, we train the base networks with Stop-C and Stop-E (240 epochs) and report the one with higher performance. To train the large network with inherited weights, we first run Alg.~\ref{alg:lottery_ticket} to obtain the `winning ticket' and then train the `winning ticket' (a small network) for 120 epochs. Then the weights of the trained `winning ticket' are loaded back to the large network to train for another 45 epochs (Stop-E) or until convergence (Stop-C). In Table~\ref{table:iwi}, the large network with inherited weights not only outperforms the `winning ticket' but also exceeds the base network.

To find out the reason, we measure the weight distributions of each network and partial results are given in Fig.~\ref{fig:weight_distribution}. It is clear that, with inherited weights as initialization, the distribution of the final weights for the large networks is sparser (closer to zero) than those with random initialization, which is in accord with Thm.~\ref{theorem:lipschitz_sparsity}. The results suggest that for networks with the same structure, IWI implicitly finds sparse weights distribution for the large networks, and the network can achieve an improved level of clean and adversarial accuracies. Moreover, it is evident that those networks are sparse and have large capacities at the same time.

Beyond performance boost, IWI also accelerates the adversarial training process, mainly due to the lower expense of adversarially training a small network, and less training epochs required after the large network inheriting weights. Details can be found in the supplementary material. We have also tried other methods, such as using an additional regularization term to impose sparsity in large networks, but it failed. Interested readers may refer to the supplementary material for more details.
%However, a large network may also be sparser (besides $L_0 sparsity$) to achieve higher robustness as we analyze in \ref{section:story_1}. Interestingly, we show the point in \cite{DBLP:conf/iclr/MadryMSTV18} is still valid despite the success of adversarial network pruning, by introducing a new training strategy called inverse weights inheritance. Our training strategy is motivated by: the pruned and well-retrained network may provide the large network with important weights and high sparsity, after retraining, the large network may obtain a sparser weights distribution than a normally adversarially trained one.

\iffalse
\YE{Above the performance boost and acceleration for adversarial training, we also found that the pruned network obtained by IWI was more robust than the state-of-the-art methods for model compression for adversarial robustness---adversarial training model compression method (ATMC, \cite{gui2019model}). We have achieved 71.14\% adversarial accuracy against the PGD-7 attack which is more than 30\% higher than the results reported in \cite{gui2019model}. This shows a practical application for lottery ticket hypothesis to compress models without hurting their adversarial robustness.}
\fi

%We also tried penalty such as $L_2$-regularization to make the network sparser (see supplementary material), as indicated in \cite{DBLP:journals/corr/GoodfellowSS14}, this fail to improve robustness.



==> LaTeX arXiv/story/lottery.tex <==
\begin{algorithm}[!b]
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\caption{Lottery Ticket in Adversarial Settings}
	\fontsize{9.5pt}{10.5pt}\selectfont
	\label{alg:lottery_ticket}
	\begin{algorithmic}[1] %[1] enables line numbers
		\REQUIRE A large network $ f \left(x;\theta_0\odot M_0\right)$ where $x$ is the input, $\theta_0$ is the randomly initialized weights, and $M_0=1^{|\theta_0|}$ denoting weight masks. \\
		~~~~~ Iterative pruning ratio $ p\% $. \\
		~~~~~ Pruning iteration $ K $. \\
		~~~~~ Training epochs $ N $ per pruning iteration. \\
		\ENSURE A winning ticket $ f \left(x;\theta_0\odot M_K\right) $.
		%        \STATE Conduct iterative pruning with parameters $\{ p\%, K, N \}$ on $f$ and find its `winning ticket' $g \left(x; \theta_0\odot M' \right)$ where $ M'[i]=0 $ if $ \theta_0[i] $ is pruned.
		\FOR{k in $ \left\{1,\dots,K\right\} $}
		\STATE {Conduct adversarial training on $ f \left(x;\theta_{0} \odot M_{k-1}\right)$ for $ N $ epochs and obtain the network $ f \left(x;\theta_k\odot M_{k-1}\right)$.}
		\STATE {Prune $ p\% $ weights from the current network and obtain a new weights mask $ M_k $.}
		\STATE {Re-initialize weights of $ f $ as $ f \left(x;\theta_0\odot M_k\right) $.}
		\ENDFOR
		\STATE{\textbf{return} $ f \left(x;\theta_0\odot M_K\right) $.}
	\end{algorithmic}
\end{algorithm}

\input{tables/lottery_ticket100}

\input{tables/iwi100}

\subsection{Lottery Tickets in Adversarial Settings}

We seek that in a randomly-initialized large network, if a subnetwork exists achieving comparable robustness as the large one, which is also known as the `winning ticket' in \citet{DBLP:conf/iclr/FrankleC19} in a natural setting. More specifically, we perform Alg.~\ref{alg:lottery_ticket} to find out the `winning ticket' in the adversarial setting. A discussion of hyperparameters can be found in the supplementary material. 

% \input{tables/lottery_ticket100}

The results on CIFAR-10 and CIFAR-100 are displayed in Table~\ref{table:lottery_ticket}. We mark the results with comparable performance to the base large networks in bold. On ResNet18 and VGG16 trained on CIFAR-10, no noticeable performance degradation occurs when the pruning ratio is as high as $ 80\% $. This is slightly different from pruning on natural models \cite{DBLP:conf/iclr/FrankleC19}, where accuracies do not drop until pruning ratio reaches around $ 88.2\% $ and $ 92 \% $ respectively on Resnet18 and VGG16. We think the difference may be explained by the more complicated decision boundary of a robust model (in theory, a model with a higher Rademacher complexity is needed to achieve adversarial robustness), and hence its `winning ticket' requires a higher capacity.

To better understand lottery tickets in adversarial settings, we compare the weights distribution between one-shot pruned model and the winning ticket at the same pruning ratio. Fig.~\ref{fig:lottery_gup} illustrates the example of two models pruned at the same pruning ratio by GUP and Alg.~\ref{alg:lottery_ticket} respectively on CIFAR10, with adversarial accuracy 47.09\% versus 47.36\% on ResNet18, and 44.36\% versus 45.15\% on VGG16, correspondingly. 
As we observe, whereas GUP models tend to have a flatter distribution which is consistent with \citet{DBLP:journals/corr/abs-1903-12561}, the winning tickets have more near-zero valued weights, indicating a higher level of sparsity. Thus we conclude that it is able to achieve preferable adversarial robustness through the lottery tickets settings. 
\begin{figure}[h]
	\centering
	\includegraphics[width=\columnwidth]{figures/lottery_gup.pdf}
	\caption{Weights distribution example of the pruned network obtained by one-shot \textbf{GUP} and \textbf{adversarial lottery} at the same pruning ratio. Note that we have a logarithmic y-axis such that the near-zero values are highly dense in the upper part of the figure. The distribution indicates that the adversarial winning tickets have higher sparsity than corresponding GUP pruned models. }
	\label{fig:lottery_gup}
\end{figure}

\subsubsection{Comparison with previous results.}
\citet{DBLP:journals/corr/abs-1903-12561} argues against the existence of `winning ticket' in adversarial settings. Nevertheless, through experiments we show that `winning ticket' exists in adversarial settings and can be obtained efficiently with a few rounds of pruning and less retraining. Our conclusion is different mostly because we search `winning ticket' by iterative global unstructured pruning as in \citet{DBLP:conf/iclr/FrankleC19}, while \citet{DBLP:journals/corr/abs-1903-12561} uses a layer-wise pruning method. As indicated in \citet{DBLP:conf/iclr/FrankleC19}, layers with fewer parameters may become bottlenecks under a layer-wise pruning method, and thus winning tickets fail to emerge. We also compare our work with \citet{li2020towards}, and find the few-shot pruning in \citet{li2020towards} does not outperform iterative pruning results in our setting. 
% Evaluation and comparison of these results under PGD iterations 10 and 7 for training and testing, respectively, can be found in supplementary materials. 

We also plot the results in Table \ref{table:advcom_three_datasets} and Table \ref{table:lottery_ticket} by showing the relation between the number of parameters of the pruned models against the adversarial accuracy in Fig.~\ref{fig:nparam}. By comparing with recent works including RobNet \cite{Guo2020} and ATMC \cite{gui2019model} utilizing the same training and testing metrics, which is PGD10 and PGD100, respectively, we demonstrate that our approach are able to acquire smaller networks with robustness comparable to the original dense models through adversarial network pruning, extensively effective under different current model structures among ResNet, VGG, and DenseNet. 

==> LaTeX arXiv/story/theory.tex <==
% \subsection{Sparsity and Robustness}

In this section, we theoretically prove that sparser weights distribution indicates an improved level of robustness. In the theoretical deduction, we assume DNNs with ReLU activation functions, but the conclusion can be generalized to a variety of models, as we verify by experiments.

%By extending the theoretical work in \cite{guo2018sparse} to other kinds of sparsity, we find higher robustness of networks inheriting weights can be explained by their higher $L_p$-sparsity. We mainly focus on nonlinear DNNs with ReLU activation function.
We focus on nonlinear DNNs with ReLU activation functions for classification tasks as an example to study the connection between sparsity and robustness. Let us consider a multi-layer perceptron $g\left(\cdot\right)$ trained with labeled training datasets $\{\left(x_i, y_i\right)\}$. Each layer of the network is parameterized by a weight matrix $ W_d \in \mathbb{R}^{n_{d-1}\times n_d} $ and $ w_k = W_d[:,k]$ represents the weights associated with the $k$-th class in the final layer. $ \sigma $ denotes the ReLU function. Then the prediction scores of $x_i$ for class $k$ can be denoted as
\begin{equation}
\label{equation:perceptron}
g_k\left(x_i\right) = w_k^T \sigma \left(W_{d-1}^T \sigma \left( ... \sigma \left( W_1^T x_i \right) \right) \right).
\end{equation}
Let $\hat{y}=\arg\max_{k\in\{1,...,c\}}g_k\left(x\right)$ denote the class with the highest prediction score.  Assuming the classifier is Lipschitz continuous, the local Lipschitz constant of function $g_{\hat{y}}\left(x\right)-g_k\left(x\right)$ over the neighborhood of $x$ is defined as $ L^k_{q,x} = \max_{x \in B_p\left(0,R\right)} \Vert \nabla g_{\hat{y}}(x)-\nabla g_k(x) \Vert$, where $B_p\left(x,R\right)$ denotes a ball centered at $x$ with radius $R$ under $L_p$ norm. Previous works \cite{hein2017formal,guo2018sparse} have associated robustness with the local Lipschitz constant by the following theorem:
\begin{theorem}
	\label{theorem:robustness_guarantee}
	\cite{hein2017formal,guo2018sparse} Let $\hat{y}=\arg\max_{k\in\{1,...,c\}}g_k\left(x\right)$ and $\frac{1}{p}+\frac{1}{q}=1$. For any perturbation $\delta_x\in B_p\left(0,R\right)$, $p \in \mathbb{R}^+$ and a set of Lipschitz continuous functions $\{g_k:\mathbb{R}^n\mapsto\mathbb{R}\}$, the classification decision on $x'$ will not change with
	\begin{equation}
	\label{equation:robustness_guarantee}
	\left\Vert\delta_x\right\Vert_p \le \min\left\{ \min_{k\ne\hat{y}} \frac{g_{\hat{y}}\left(x\right)-g_k\left(x\right)}{L^k_{q,x}}\right\},
	\end{equation}
	where $ L^k_{q,x} = \max_{x' \in B_p\left(0,R\right)} \Vert \nabla g_{\hat{y}}(x')-\nabla g_k(x') \Vert$.
\end{theorem}

Eqn.~\eqref{equation:robustness_guarantee} has clearly depicted the relation between robustness and the local Lipschitz constant --- a smaller $L^k_{q,x}$ represents a higher level of robustness as a larger distortion can be tolerated without changing the prediction. \citet{guo2018sparse} further gives the relation between the local Lipschitz constant and the weights. We further deduct that the relation satisfies the following theorem:
\begin{theorem}
	\label{theorem:lipschitz_sparsity}
	(The robustness and weights distribution of ReLU networks.) Letting $\frac{1}{p}+\frac{1}{q}=1$, for any $x \in \mathbb{R}^n $, $k \in \{1,...,c\}$ and $q \in \{1,2\}$, the local Lipschitz constant of function $ g_{\hat{y}}\left(x\right)-g_k\left(x\right) $ satisfies
	\begin{equation}
	\label{equation:lipschitz_sparsity}
	L^k_{q,x} \le \left\Vert w_{\hat{y}}-w_k \right\Vert_q
	\prod_{j=1}^{d-1}\left({\left\Vert W_j \right\Vert_p} \right).
	\end{equation}
\end{theorem}
Note that the local Lipschitz constant is upper bounded by the product of the $L_{p}$-norm of the weights matrices. That is to say, if $\left\Vert W_j \right\Vert_p$ is small, $L^k_{q,x}$ is constrained to be small, leading to a higher level of robustness. The proof of Thm.~\ref{theorem:lipschitz_sparsity} is omitted here due to space constraint and we refer readers to the supplementary document for the detailed proof.

We have at least two interpretations of Thm.~\ref{theorem:lipschitz_sparsity}: if we let $p=0$, Eqn.~\eqref{equation:lipschitz_sparsity} is bounded by the number of non-zero weights of the model, and hence the higher the proportion of non-zero weights, the more robust the model is. On the other hand, a smaller value of $\left\Vert W_j \right\Vert_p$ suggests the distribution of weights is closer to zero. This indicates that if a model has a weights distribution closer to zero, it may be more robust than other models with the same structure. We will respectively show how the two points are supported by the experimental results.



==> LaTeX arXiv/tables/advcom_three_datasets100.tex <==
\begin{table*}[!t]
%\begin{wraptable}{r}{10cm}
	\centering
	\caption{\textbf{Clean testing accuracy/adversarial testing accuracy (in \%)/distortion lower bound} of pruned networks with adversarial retraining. Accuracy and distortion bounds higher than the base model are in bold.}
	\fontsize{9pt}{10pt}\selectfont
	\begin{subtable}[c]{\linewidth}
		\centering
% 		\resizebox{1.\textwidth}{!}{
			\begin{tabular}{@{}cccccc@{}}
				\toprule
				\multicolumn{6}{c}{\textbf{(a)   } One-Shot Pruning on CIFAR-10 w/ Stop-E} \\ \toprule
				Network                                                                           & $p\%$ & LUP & GUP & FP & NS \\ \midrule
				\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ResNet18\\ (82.84/49.40/2.519)\end{tabular}}
				& 30  & \textbf{82.13/49.9/3.221}    & \textbf{81.92}/46.56/2.402   & \textbf{83.62}/46.61/2.505   & \textbf{84.18/49.92}/2.023      \\
				& 60  & 82.21/48.44/\textbf{2.777}   & \textbf{84.73/49.64/2.612}   & 82.61/48.08/2.501   & \textbf{83.57/49.46/2.666}      \\
				& 90  & 80.09/46.76/1.533            & \textbf{83.89}/47.09/\textbf{2.940}  & 78.87/46.24/1.764   & -                \\ \midrule
				\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}VGG16\\ (78.57/44.68/3.471)\end{tabular}}
				& 30  & \textbf{79.81}/43.17/1.982  & \textbf{80.43}/44.24/1.630    & 77.05/43.91/3.002   & \textbf{80.10}/43.81/2.991       \\
				& 60  & \textbf{78.78}/43.30/2.136  & \textbf{80.26}/43.51/2.275    & 77.13/44.21/2.032   & \textbf{79.56}/44.29/2.607      \\
				& 90  & 72.1/41.98/2.510            & \textbf{79.83}/44.36/2.501    & 69.38/41.20/2.270   & \textbf{79.54}/43.76/2.443      \\ \midrule
				\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}DenseNet-BC\\ (76.01/44.26/1.109)\end{tabular}}
				& 30  & 74.42/43.76/\textbf{1.525}  & 74.68/43.40/\textbf{2.928}   & -             & 73.86/43.08/\textbf{2.572}              \\
				& 60  & 73.16/42.70/\textbf{1.734}  & 73.24/42.88/\textbf{1.781}   & -             & 66.33/37.54/1.059              \\
				& 90  & 63.15/36.68/\textbf{2.000}  & 65.19/36.85/\textbf{1.784}   & -             & -              \\ \bottomrule
			\end{tabular}
% 		}
	\end{subtable}
% 	\\
	\begin{subtable}[c]{.9\linewidth}
		\centering
% 		\resizebox{1.\textwidth}{!}{
			\begin{tabular}{@{}cccccc@{}}
				\toprule
				\multicolumn{6}{c}{\textbf{(b)   } One-Shot Pruning on Tiny-ImageNet w/ Stop-C} \\ \toprule
				Network                                                                           & $p\%$ & LUP    & GUP   & FP          & NS          \\ \midrule
				\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ResNet18\\ (41.94/14.43/2.594)\end{tabular}}
				& 30  & \textbf{42.72/14.87}/2.356 & \textbf{43.18/15.82/2.713} & \textbf{42.68/14.91/3.300} & \textbf{41.89/15.23}/2.397 \\
				& 60  & \textbf{42.28/15.51/3.022} & \textbf{42.80/16.12/3.272} & 40.88/\textbf{15.87}/1.172 & 37.92/14.11/\textbf{3.250} \\
				& 90  & 40.32/\textbf{16.11}/2.581 & \textbf{42.21/17.26/2.797} & 36.79/14.43/1.819 & -         \\ \midrule
				\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}DenseNet121\\ (49.48/19.65/1.922)\end{tabular}}
				& 30  & \textbf{48.86/20.03/3.616}   & \textbf{48.19/20.52/2.519} & -  & 46.43/\textbf{19.71}/1.597        \\
				& 60  & \textbf{48.63/19.98/2.300} & \textbf{48.96/19.92/1.984} & -           & 40.82/16.51/\textbf{3.334}         \\
				& 90  & 45.72/18.75/1.722         & 46.99/18.65/1.478 & -           & -
				\\ \bottomrule
			\end{tabular}
% 		}
		%\caption{\textbf{Tiny-ImageNet} with \textbf{Expense-C}}
		%\label{table:advcom_Tiny-ImageNet_expense_c}
	\end{subtable}
	\label{table:advcom_three_datasets}
%\end{wraptable}
\end{table*}


==> LaTeX arXiv/tables/compare_prune_and_scratch100.tex <==
\begin{table}[!t]
	\centering
	\caption{\textbf{Clean testing accuracy/adversarial testing accuracy} (in \%) of scratch networks that shares the same structure with the corresponding pruned network, only with the weights randomly initialized. Accuracy and distortion bounds higher than the base model are in bold.}
	\fontsize{9pt}{10pt}\selectfont
% 	\resizebox{1.\textwidth}{!}{
		\begin{tabular}{@{}c@{~}c@{~}c@{~~}c@{~~}c@{~~}c@{}}
			\toprule
			\multicolumn{6}{c}{\begin{tabular}[c]{@{}c@{}}One-Shot Pruning w/ Randomly Initialized Weights\\on CIFAR-10 w/ Stop-E\end{tabular}}                                                                                                                                                                    \\ \toprule
			Network                   & $ p\% $ & LUP-rand             & GUP-rand   & FP-rand            & NS-rand     \\ \midrule
% 			\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ResNet18\\ (82.84/50.87)\end{tabular}}
			\multirow{3}{*}{ResNet18}
			& 30  & 81.91/46.54  & 81.41/48.78  & 82.24/46.58  & \textbf{83.21}/46.28 \\
			& 60  & 82.58/46.40  & 81.91/47.46  & 80.64/46.22  & 82.61/46.04 \\
			& 90  & 78.36/44.97  & 81.99/46.90  & 80.34/45.50  & - \\ \midrule
% 			\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}VGG16\\ (78.57/48.04)\end{tabular}}
			\multirow{3}{*}{VGG16}
			& 30  & \textbf{79.67}/42.37  & \textbf{79.56/45.26}  & \textbf{80.27}/44.38  & \textbf{78.68}/43.52 \\
			& 60  & 78.26/43.79  & \textbf{80.23/45.22}  & 78.52/44.21  & \textbf{78.77}/43.74 \\
			& 90  & 72.32/41.38  & 77.78/43.97  & 74.24/42.39  & 77.37/43.52 \\ \bottomrule
		\end{tabular}
% 	}
	\label{table:compare_prune_and_scratch}
\end{table}


==> LaTeX arXiv/tables/iwi100.tex <==
\begin{table*}[!t]
	\centering
	\caption{\textbf{Clean testing accuracy/adversarial testing accuracy (in \%)/distortion lower bound}. Performance of base networks are marked under the model name. The performance of the inherited Winning Tickets is shown in Table~\ref{table:lottery_ticket}. Performance higher than the base model is in bold.}
	\fontsize{9pt}{10pt}\selectfont
% 	\resizebox{1.\textwidth}{!}{
		\begin{tabular}{@{}cccc|cccc@{}}
			\toprule
			\multicolumn{4}{c}{\textbf{(a)} Inverse Weights Inheritance on CIFAR-10}  &\multicolumn{4}{|c}{\textbf{(b)} Inverse Weights Inheritance on CIFAR-100}\\ \toprule
			Network & $p\%$ & Stop-C & Stop-E  & Network & $p\%$ & Stop-C & Stop-E         \\ \midrule
			\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}ResNet18\\ 82.84/49.40/2.519 \end{tabular}}
			& 80  & \textbf{84.05/50.30/2.728}   & \textbf{83.14/49.59}/2.303
			& \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}ResNet18\\ 50.50/21.13/3.047\end{tabular}}
			& 30  & \textbf{53.49/22.07/3.872} & \textbf{51.57}/20.68/1.191\\
			& 90  & \textbf{83.56/49.89/2.819}   & 81.68/49.03/\textbf{2.662}  & & 60  & \textbf{52.98/21.65/3.197} & \textbf{50.74/21.28/3.472}\\
			& 95  & \textbf{84.60}/49.34/\textbf{2.659}   & \textbf{83.19}/48.93/1.734  & & 80  & 50.06/21.03/1.900 & \textbf{50.78/21.15}/1.881\\
			& -   & -                            & -                           & & 90  & \textbf{52.91/21.53}/2.812 & 50.16/\textbf{21.39}/2.056\\
			\midrule
			\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}VGG16\\ 78.57/44.68/3.471 \end{tabular}}
			& 80  & \textbf{81.21/47.38}/2.338   & \textbf{81.15/47.46}/1.600
			& \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}VGG16\\ 44.44/18.86/2.338\end{tabular}}
			& 30  & \textbf{47.18/18.91}/1.491          & \textbf{44.79/19.10}/1.534\\
			& 90  & \textbf{81.36/47.54}/2.597   & \textbf{80.74/47.53}/2.622  & & 60  & \textbf{45.97/19.38}/1.147          & \textbf{45.16}/18.68/1.191\\
			& 95  & \textbf{81.29/46.98}/3.341   & \textbf{80.68/47.59}/3.219  & & 80  & \textbf{46.51/19.22/2.631}          & 43.79/\textbf{18.90/2.759}\\
			& -   & -                            & -                           & & 90  & \textbf{47.64/19.26/3.169} & 43.30/\textbf{18.94}/2.000\\
			\bottomrule
		\end{tabular}
% 	}
	\label{table:iwi}
% 	\vspace{-3mm}
\end{table*}


==> LaTeX arXiv/tables/lottery_ticket100.tex <==
\begin{table}[!t]
	\centering
	\caption{\textbf{Clean testing accuracy/adversarial testing accuracy} (in \%) of adversarially trained `winning ticket.' $p\%$ is the pruning ratio. `60 ($ 20\times \text{3 iter} $)' means iteratively remove $20\%$ of the weights in each for 3 iterations to achieve a final pruning ratio of $60\%$. Each iteration of pruning is preceded by 1 epoch of training, and the total training epoch is 240. Accuracy and distortion bounds higher than the base model are in bold. }
	\fontsize{9pt}{10pt}\selectfont
% 	\resizebox{1.\textwidth}{!}{
		\begin{tabular}{@{}cccc@{}}
			\toprule
			\multicolumn{4}{c}{ Winning Tickets on CIFAR-10 and CIFAR-100 w/ Stop-E }   \\ \toprule
			Network & $p\%$ & CIFAR-10            & CIFAR-100 \\ \midrule
			\multirow{6}{*}{ResNet18}
			& 0 (baseline) & 82.84/49.40 & 50.50/21.13 \\
			& 30 ($ 30\times \text{1 iter} $) & \textbf{84.29}/45.54 & \textbf{50.62/21.72} \\
			& 60 ($ 20\times \text{3 iter} $) & \textbf{84.03}/47.99 & \textbf{52.68/21.54}  \\
			& 80 ($ 20\times \text{4 iter} $) & \textbf{81.41}/48.19 & \textbf{52.23}/20.80  \\
			& 90 ($ 30\times \text{3 iter} $) & 70.29/47.36 & 49.43/21.27 \\
			& 95 ($ 31.7\times \text{3 iter} $) & 70.29/39.35 & - \\ \midrule
			\multirow{6}{*}{VGG16}
			& 0 (baseline) & 78.57/44.68 & 44.44/18.86 \\
			& 30 ($ 30\times \text{1 iter} $) &  \textbf{80.90/45.58} & 42.21/\textbf{19.16} \\
			& 60 ($ 20\times \text{3 iter} $) &  \textbf{80.05/45.56} & 42.65/\textbf{19.12}  \\
			& 80 ($ 20\times \text{4 iter} $) &  \textbf{79.30/45.16} & 45.90/\textbf{18.93}  \\
			& 90 ($ 30\times \text{3 iter} $) &  \textbf{78.87/45.15} & 45.76/\textbf{18.89} \\
			& 95 ($ 31.7\times \text{3 iter} $) & 68.48/40.10 & -  \\
			\bottomrule
		\end{tabular}
% 	}
	\label{table:lottery_ticket}
\end{table}

% Backup
\iffalse
\begin{table*}[t]
	\centering
	\caption{\textbf{Clean testing accuracy/adversarial testing accuracy (sum of both)} (in \%) of adversarially trained `winning ticket.' $p\%$ is the pruning ratio. `60 ($ 20\times \text{3 iter} $)' means we iteratively remove $20\%$ of the weights in each iteration for 3 iterations to achieve a final pruning ratio of $60\%.$ Each iteration of pruning is preceded by 1 epoch of training. Each model is run for a total of 240 epochs. The total accuracies (clean accuracy plus adversarial accuracy) within $ 0.5\%$ loss compared to the base model are marked in bold. }
	\fontsize{9pt}{10pt}\selectfont
% 	\resizebox{1.\textwidth}{!}{
		\begin{tabular}{@{}c|ccc|ccc@{}}
			\toprule
			\multicolumn{7}{c}{ Training Winning Tickets w/ Stop-E }   \\ \toprule
			$p\%$ & Network                   & CIFAR-10            & CIFAR-100              &
			Network                   &  CIFAR-10             & CIFAR-100              \\ \midrule
			0 &\multirow{5}{*}{ResNet18} & 82.84/50.87 & 50.50/21.71 &
			\multirow{5}{*}{VGG16}    & 78.57/48.04 & 44.44/19.29 \\
			30 ($ 30\times \text{1 iter} $)  & & \textbf{83.34/51.20} & \textbf{50.62/21.42} &
			&  \textbf{80.34/48.26} & 42.21/19.68 \\
			60 ($ 20\times \text{3 iter} $) & & \textbf{82.14/51.26} & \textbf{52.68/19.26} &
			&  \textbf{79.36/47.86} & 42.65/19.49 \\
			80 ($ 20\times \text{4 iter} $) & & \textbf{84.02/49.36} & \textbf{52.23/20.48} &
			&  \textbf{80.60/46.06} & 45.90/16.43 \\
			90 ($ 30\times \text{3 iter} $) & & 82.57/48.99 & 49.43/21.06 &
			& 80.00/45.80 & 45.76/17.39 \\
			95 ($ 31.7\times \text{3 iter} $) & & 70.29/40.68 & - &
			& 68.48/40.77 & -          \\
			\bottomrule
		\end{tabular}
% 	}
	\label{table:lottery_ticket}
\end{table*}
\fi

\iffalse
\begin{table*}[t]
	\centering
	\caption{\textbf{Clean testing accuracy/adversarial testing accuracy (sum of both)} (in \%) of adversarially trained `winning ticket.' $p\%$ is the pruning ratio. `60 ($ 20\times \text{3 iter} $)' means we iteratively remove $20\%$ of the weights in each iteration for 3 iterations to achieve a final pruning ratio of $60\%.$ Each iteration of pruning is preceded by 1 epoch of training. Each model is run for a total of 240 epochs. The total accuracies (clean accuracy plus adversarial accuracy) within $ 0.5\%$ loss compared to the base model are marked in bold. }
	\resizebox{1.\textwidth}{!}{
		\begin{tabular}{@{}c|ccc|ccc@{}}
			\toprule
			\multicolumn{7}{c}{ Training Winning Tickets w/ Stop-E }   \\ \toprule
			$p\%$ & Network                   & CIFAR-10            & CIFAR-100              &
			Network                   &  CIFAR-10             & CIFAR-100              \\ \midrule
			0 &\multirow{5}{*}{ResNet18} & 82.84/50.87(133.71)           & 50.50/21.71(72.21)          &
			\multirow{5}{*}{VGG16}    & 78.57/48.04(126.61)          & 44.44/19.29(63.73)          \\
			30 ($ 30\times \text{1 iter} $)  &                           & \textbf{83.34/51.20(134.54)} & \textbf{50.62/21.42(72.04)} &
			&  \textbf{80.34/48.26(128.60)} & 42.21/19.68(61.89)          \\
			60 ($ 20\times \text{3 iter} $) &                           & \textbf{82.14/51.26(133.40)} & \textbf{52.68/19.26(71.94)} &
			&  \textbf{79.36/47.86(127.22)} & 42.65/19.49(62.14)          \\
			80 ($ 20\times \text{4 iter} $) &                           & \textbf{84.02/49.36(133.38)} & \textbf{52.23/20.48(72.71)} &
			&  \textbf{80.60/46.06(126.66)} & 45.90/16.43(62.33)          \\
			90 ($ 30\times \text{3 iter} $) &                           & 82.57/48.99(131.56)          & 49.43/21.06(70.49)          &
			& 80.00/45.80(125.80)          & 45.76/17.39(63.15)          \\
			95 ($ 31.7\times \text{3 iter} $) &                           & 70.29/40.68(110.97)        & -          &
			& 68.48/40.77(109.25)          & -          \\
			\bottomrule
		\end{tabular}
	}
	\label{table:lottery_ticket}
\end{table*}
\fi


==> Proof.tex <==
\section{Proof of Theorem 3.2}
	Let us denote layer-wise activation output as $ a_0=x $ and $ a_j = \sigma \left( W_j^T a_{j-1} \right) $ for $ 0 \le j \le d-1 $. We also define $ D_j $ as
    \begin{equation}
        \label{equation:activation}
            D_j\left(x\right) := diag \left( 1_{W_j[:,1]^T a_{j-1}>0}, ..., 1_{W_j[:,n_j]^T a_{j-1}>0} \right)
    \end{equation}
    which is a diagonal matrix whose entries will take value one when the activation is nonzero within $j$-th layer. Note that if for any $x$ and any $j \in \{1,...,d-2\}$, $D_j(x)=0^{n_j \times n_j}$, $D_{d-1}(x)=0^{n_{d-1} \times n_{d-1}}$ must hold. In this setting, we have Lemma \ref{lemma:lipschitz_sparsity_with_D} proved by \cite{guo2018sparse}.

    \begin{lemma}
        \label{lemma:lipschitz_sparsity_with_D}
        (A local Lipschitz constant for ReLU networks \cite{guo2018sparse}) Letting $\frac{1}{p}+\frac{1}{q}=1$, for any $x \in \mathbb{R}^n $, $k \in \{1,...,c\}$ and $q \in \{1,2\}$, the local Lipschitz constant of function $ g_{\hat{y}}\left(x\right)-g_k\left(x\right) $ satisfies
        \begin{equation}
        \label{equation:lipschitz_sparsity_with_D}
            L^k_{q,x} \le \left\Vert w_{\hat{y}}-w_k \right\Vert_q\sup_{x'\in B_p\left(x,R\right)}\prod_{j=1}^{d-1}
            \left( {\left\Vert D_j\left(x'\right) \right\Vert_p} {\left\Vert W_j \right\Vert_p} \right)
        \end{equation}
        where all the matrix norms are induced norms.
    \end{lemma}

    In our settings, the network is pruned to avoid layer removal and thereby for any $j \in [0, d-1]$, $W_{j}$ cannot be all-zero matrices. Then we prove for any $j \in [0, d-1]$, there must be at least one $a_{j}$ which is not an all-zero matrix. We prove that by contradiction. Assume that for layer $j$, $a_{j}$ is an all-zero matrix. Then $D_{j}(x) = 0^{n_{d-1} \times n_{d-1}}$ which yields $D_{d-1}(x)=0^{n_{d-1} \times n_{d-1}}$ and the prediction score $g_k(x)$ will be all-zero for any $k$ since 
    \begin{equation}
        \label{equation:perceptron}
            g_k\left(x_i\right) = w_k^T \sigma \left(W_{d-1}^T \sigma \left( ... \sigma \left( W_1^T x_i\right) \right) \right).
    \end{equation}
    It is impossible for a well-trained network to make all-zero predictions, which leads to a contradiction. Hence the assumption is not true and $a_{j}, \forall j\in [0, d-1] $ cannot be an all-zero matrix. The conclusion implies that, for any $j\in [0, d-1]$, there must be at least one entry in $ D_{j}(x) $ taking the value $1$. By the definition of matrix induced norms, we have that for any $x$ and particular values of $p$,
    \begin{equation}
        \label{equation:L_2_norm}
        \left\Vert D_j\left(x\right) \right\Vert_2 := \sigma_{\max}(D_j) = 1
    \end{equation}
    \begin{equation}
        \label{equation:L_inf_norm}
        \left\Vert D_j\left(x\right) \right\Vert_\infty := \max_{1\le i \le n_j}\sum_{m=1}^{n_j}\vert D_j[i,m]\vert = 1
    \end{equation}
    where $\left\Vert D_j\left(x\right) \right\Vert_2$ is the spectral norm, the greatest singular value of $D_j\left(x\right)$. Then for $p = 2$ and $\infty$, the right side of Eq.~\eqref{equation:lipschitz_sparsity_with_D} is independent of input $ x $ and we have the relation between the Lipschitz constant and weight sparsity described by Theorem 3.2.
